Unsupervised Text Style Transfer via LLMs and Attention Masking with Multi-way Interactions

Unsupervised Text Style Transfer (UTST) has emerged as a critical task within the domain of Natural Language Processing (NLP), aiming to transfer one stylistic aspect of a sentence into another style without changing its semantics, syntax, or other attributes. This task is especially challenging given the intrinsic lack of parallel text pairings. Among existing methods for UTST tasks, attention masking approach and Large Language Models (LLMs) are deemed as two pioneering methods. However, they have shortcomings in generating unsmooth sentences and changing the original contents, respectively. In this paper, we investigate if we can combine these two methods effectively. We propose four ways of interactions, that are pipeline framework with tuned orders; knowledge distillation from LLMs to attention masking model; in-context learning with constructed parallel examples. We empirically show these multi-way interactions can improve the baselines in certain perspective of style strength, content preservation and text fluency. Experiments also demonstrate that simply conducting prompting followed by attention masking-based revision can consistently surpass the other systems, including supervised text style transfer systems. On Yelp-clean and Amazon-clean datasets, it improves the previously best mean metric by 0.5 and 3.0 absolute percentages respectively, and achieves new SOTA results.

==> exp_backup_data.tex <==
% \yscomment{We can find if there are other datasets that our systems can defeat other systems generally.}
% \begin{table}[htbp]
% \centering
% \caption{Performance of different models on various datasets.}
% \begin{tabular}{@{}lccllccllllll}
% \toprule
% Model & \multicolumn{2}{c}{Amazon} &  && \multicolumn{2}{c}{Yelp} & & & Politeness & & &\\
% \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7}& ACC & s-BLEU  & r-BLEU&PPL& ACC & s-BLEU    &r-BLEU& PPL& ACC & s-BLEU    & r-BLEU&PPL\\
% \midrule
% DRG\cite{li2018delete} & 52.2\% & 57.89 $\pm$ 2.19  & 32.47 ± 12.68&& 84.1\% & 32.18 $\pm$ 2.05    && & & & &\\
% StyTrans\cite{dai2019style} & 67.8\% & 82.07 $\pm$ 1.56  & 32.88 ± 2.47&& 92.1\% & 52.40 $\pm$ 2.14    && & & & &\\
% DGST \cite{li2020dgst}& 59.2\% & 83.02 $\pm$ 1.25  &  42.20 ± 22.37&& 88.0\% & 51.77 $\pm$ 2.41    && & & & &\\
% TAG \cite{madaan2020politeness} & 79.4\% & 58.13 $\pm$ 1.46  & 25.95 ± 1.86&& 88.6\% & 47.14 $\pm$ 2.23    && & & & &\\
% DIRR \cite{liu-2022-low} & 62.7\% & 66.63 $\pm$ 2.51  & 32.68 ± 2.25&& 91.2\% & 56.56 $\pm$ 1.89    && & & & &\\
% LEWIS \cite{reid2021lewis} & 71.8\% & 65.53 $\pm$ 1.44  & 30.61 ± 1.57&& 89.4\% & 54.67 $\pm$ 1.62    && & & & &\\
% MAR \cite{yang2022mask}& \textbf{80.2\%} & \textbf{83.42 $\pm$ 1.46}  & && \textbf{93.9\%} & \textbf{53.32 $\pm$ 1.86}    && & & & &\\
% \bottomrule
%  EPAAE \cite{narasimhan2022towards}& &  & && 77.1\%&   && & & & &\\
%  GPT-3.5 \cite{yerukola2023don}& &  & && 70\%&   && 48& & & &\\
%  STEC \cite{zhu2022slow}& 66.2&  67.1& 36.5&& 88.6\%&   60.2&21.7& & 88.9& 68.7& &\\
%  SA-MLM\cite{narasimhan2023text}& 63.9& 29.6& 69.8& & 91.2& 18.3&  53.4& & & & &\\
% \end{tabular}
% \label{tab:my_label}
% \end{table}





% \begin{table*}[htbp] % Notice the use of table* instead of table
% \centering
% \caption{Performance of different models on various datasets.}
% {\tiny
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccc@{}}
% \toprule
% Model & \multicolumn{3}{c}{Amazon} & \multicolumn{3}{c}{Yelp} & \multicolumn{2}{c}{IMDb} \\
% \cmidrule(r){2-4} \cmidrule(lr){5-7} \cmidrule(l){8-9}
%  & ACC & s-BLEU & r-BLEU & ACC & s-BLEU & r-BLEU & ACC & s-BLEU \\
% \midrule
% DRG\cite{li2018delete} & 52.2\% & 57.89 $\pm$ 2.19 & 32.47 $\pm$ 12.68 & 84.1\% & 32.18 $\pm$ 2.05 & 12.28 $\pm$ 1.33 & 55.8\% & 55.40 $\pm$ 1.79 \\
% StyTrans\cite{dai2019style} & 67.8\% & 82.07 $\pm$ 1.56 & 32.88 $\pm$ 4.17 & 92.1\% & 52.40 $\pm$ 2.14 & 19.91 $\pm$ 2.01 & 86.6\% & 66.20 $\pm$ 1.55 \\
% DGST \cite{li2020dgst} & 59.2\% & 83.02 $\pm$ 1.25 & 42.20 $\pm$ 22.37 & 88.0\% & 51.77 $\pm$ 2.41 & 19.05 $\pm$ 1.89 & 70.1\% & 70.20 $\pm$ 1.42 \\
% TAG \cite{madaan2020politeness} & 79.4\% & 58.13 $\pm$ 1.46 & 25.95 $\pm$ 1.36 & 88.6\% & 47.14 $\pm$ 2.23 & 19.76 $\pm$ 1.45 & N/A & N/A \\
% DIRR \cite{liu-2022-low} & 62.7\% & 66.63 $\pm$ 2.51 & 32.68 $\pm$ 2.95 & 91.2\% & 56.56 $\pm$ 1.89 & 25.60 $\pm$ 2.33 & 83.5\% & 65.96 $\pm$ 1.12 \\
% LEWIS \cite{reid2021lewis} & 71.8\% & 65.53 $\pm$ 1.44 & 30.61 $\pm$ 1.57 & 89.4\% & 54.67 $\pm$ 1.62 & 23.85 $\pm$ 1.57 & N/A & N/A \\
% MAR \cite{yang2022mask} & \textbf{80.2\%} & \textbf{83.42 $\pm$ 1.46} & \textbf{41.21 $\pm$ 23.54} & \textbf{93.9\%} & \textbf{53.32 $\pm$ 1.86} & \textbf{22.90 $\pm$ 2.01} & \textbf{87.8\%} & \textbf{66.12 $\pm$ 1.33} \\
% EPAAE \cite{narasimhan2022towards} &  &  &  &77.1\% &  &  & & \\
% GPT-3.5 \cite{yerukola2023don}  &  &  &  & 70\%  &  &   & & \\
% STEC \cite{zhu2022slow} & 66.2\% & 67.1 & 36.5 & 88.6\% & 60.2 & 21.7 & 88.9\% & 68.7\\
% SA-MLM\cite{narasimhan2023text} & 63.9\% & 29.6 & 69.8 & 91.2\% & 18.3 & 53.4 &  & \\
% \bottomrule
% \end{tabular*}
% \label{tab:my_label}
% \end{table*}



\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/accbleu_tradeoff.png}
    \caption{ACC and \textit{s}-sBLEU of Prompt-then-AM on Yelp-clean with increasing $\alpha$.}
    \label{fig:acc_ssbleu}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/comparison_chart.png}
    \caption{ACC and PPL of Prompt-then-AM on Yelp-clean with various $\alpha$.\yscomment{Can you make Figure 2, 3 and Table 4 occupies a single row, just like Figure 3 in \url{https://aclanthology.org/2023.findings-emnlp.114.pdf}.}}
    \label{fig:acc-ppl}
\end{figure}



% \begin{table}[]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l  |c c c c c }
% \toprule
% \textbf{$\alpha$}& \textbf{Acc} (\uparrow)  & \textbf{\textit{r}-sBLEU} (\uparrow) & \textbf{\textit{s}-sBLEU} (\uparrow) & \textbf{PPL} (\downarrow) & \textbf{Mean} (\uparrow) \\
% \midrule
% %ChatGLM2 and Rerank & 0.83 & 14.7 & 20.8 & 63\\
% %Llama2 and Rerank & 0.98 & 10.2 & 13.6 & 54\\
% $\alpha = 0$& 67& 27.7& 33.1& 39& 51.9\\
% %Mask-then-Prompt-refine-ChatGLM2  & 0.79 & 30.1 & 36.4 & 57\\
% %Mask-then-Prompt-refine-llama2  & 0.80 & 24.0 & 31.0 & 50\\
% $\alpha = 0.2$& 77& 27.5& 32.6& 47& 53.0\\
% $\alpha = 0.5$& 81& $27.1$& $32.3$& $53$& 52.8\\
%  $\alpha = 0.8$& 95& 26.5& 31.1& 68& $\mathbf{54.1}$\\
% %Mask as Demo-ChatGLM2_v2.0 & 0.83 & 8.7 & 10.0 & 38\\
% %Mask as Demo-llama2_v2.0 & 0.81 & 20.5 & 24.5 & 55\\
% %LLM-as-Sign & 0.83 & 35.4 & 52.8 & 109\\
% $\alpha = 1$& $\mathbf{99}$& 26.4& 30.7& 98& 50.9\\
% % LLM-as-Sign (Llama2) & \\
% \bottomrule
% \end{tabular}
% }
% \caption{Trade-off between ACC and BLEU on Y{\small elp}-clean. References: [1] \cite{li2018delete}, [2] \cite{suzgun2022prompt} 
% }
% \end{table}



\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l l| c c c c c}
\toprule 
LLMs & Methods & \textbf{Acc} ($\uparrow$)  &	\textbf{\textit{r}-sBLEU} ($\uparrow$) &	\textbf{\textit{s}-sBLEU} ($\uparrow$) &	\textbf{PPL} ($\downarrow$) &	\textbf{Mean} ($\uparrow$)\\
\midrule
ChatGLM2& LLM-based & 67&	27.7& 33.1&	39&51.9\\
& Prompt-then-AM & 93&	26.7&	31.9&	59&$\mathbf{55.4}$\\
& AM-then-prompt & $84$&	$30.1$ &	$36.4$ &	$53$&55.2\\
% & LLM as signals & 84 &	32.6 &	39.4 &	73 &48.9\\
\midrule
GPT2-XL& LLM-based & 22 & 12.7 & 15.1 & 83 & 22.0\\
& Prompt-then-AM & 81 & 13.3 & 14.9 & 172 & 34.5\\
& AM-then-prompt & 52 & 8.4 & 9.4 & 51 & 36.0\\
% & LLM as signals & \\
\midrule
GPT-J& LLM-based & 46 & 12.8 & 28.9 & 49 & 41.0\\
& Prompt-then-AM & 87 & 12.4 & 27.6 & 78 & 48.5\\
& AM-then-prompt & 69 & 10.2 & 15.8 & 46 & 45.0\\
% & LLM as signals & \\
\bottomrule
\end{tabular}
}
\caption{A comparison of existing methods on Y{\small ELP}-clean.
}
\end{table}



%To assess the transfer strength, we focus on determining if the outputs generated by a Text Style Transfer model successfully adopt the characteristics of the intended target styles. This evaluation is conducted using a standard approach involving a classifier. Specifically, we train a binary style classifier on the relevant corpus and then use it to calculate the proportion of generated outputs that match the desired styles.

%\noindent \textbf{Content preservation.} 

%\noindent \textbf{Fluency.} We include GPT-2 to measure the smoothness and naturalness of the generated text by computing the joint probability of the sentence.


%The BLEU metric, introduced by \cite{papineni2002bleu}, is a widely recognized standard for evaluating the retention of semantic content. In our study, we employ the SacreBLEU (sBLEU) version, as proposed by \cite{post2018call}, to calculate two distinct scores: reference-BLEU (r-sBLEU) and self-BLEU (s-sBLEU). The r-sBLEU score is useful for gauging the similarity of the generated sentences to the original, ground-truth references, while the s-sBLEU score indicates the extent to which the model merely replicates the source material.

%\noindent \textbf{Fluency.} When evaluating fluency, we measure the smoothness and naturalness of the generated texts. This is done by calculating their the perplexity with the help of a pre-trained language model,  the GPT-2. It's important to note, however, that while this PPL-based method is automated and practical, it is not without its limitations, such as a tendency to favor shorter texts.

==> method_v1.0.tex <==
\subsection{Prompt-Driven Text Transformation}

The first stage of the style transfer process involves the application of a LLM to transform the original text \( T_{\text{original}} \) into the target style \( S_{\text{target}} \). This transformation is facilitated by a structured prompting technique, formulated as follows:
\begin{equation}
\begin{split}
\text{P}(T_{\text{}}, S_{\text{}}) &= \text{"Rewrite the following text in a "} \\
&\quad + S_{\text{target}} + \text{" style:} \\
&\quad + T_{\text{original}}
\end{split}
\end{equation}
In this formulation, \( T_{\text{original}} \) represents the input text in its original style, while \( S_{\text{target}} \) denotes the desired target style. The Prompt function encapsulates the structured input for the LLM.

Upon receiving this prompt, the LLM generates a new text \( T_{\text{rewritten}} \) that preserves the content of \( T_{\text{original}} \) but in the style of \( S_{\text{target}} \):
\begin{equation}
T_{\text{rewritten}} = \text{LLM}(\text{Prompt}(T_{\text{original}}, S_{\text{target}}))
\end{equation}
This stage ensures the preservation of the original content of \( T_{\text{original}} \) while adapting it to the stylistic nuances of \( S_{\text{target}} \), thereby laying the groundwork for effective style transformation.

==> method_v2.0.tex <==
\subsection{Model Overview}

We propose an approach that converts the style of a text with prompt-then-revision framework.\yscomment{Can we reverse the order of prompting and revision?}


This study presents a two-stage approach for the task of text style transfer, designed to transform text from a non-target style into a specified target style. The first stage of this method utilizes LLM to initially rewrite the text in the target style. This is achieved through a specialized prompting method that guides the LLM to apply the desired stylistic attributes to the input text. The second stage involves a refinement process, where a fine-tuned model performs detailed editing operations. This stage is crucial for enhancing the style adherence of the text, ensuring that the final output closely aligns with the target style.  In this section, we first introduce the first stage of LLM refinement, then describe how the edit method works, and finally we introduce the synthesis of stylistic data pairs.

\subsection{Prompt-Driven Text Transformation}

The foundation of our method employs prompt templates to reframe text style transfer as a natural language generation challenge. Utilizing a predefined template, we transform an input text \( T_{\text{original}} \) and its associated style transition into a natural-language prompt. This transition involves moving from the original style of \( T_{\text{original}} \) to the desired target style \( S_{\text{target}} \). 

The template, designed to encapsulate the task for the model, incorporates all necessary conditional information: the input sentence and the transition from the original style to \( S_{\text{target}} \)\yscomment{One question is that as we have already converted the style of the sentences, why should we further edit it? is it because that some expressions are neutral? But have we tried some other prompting like we show some examples of target style?}. 
\begin{equation}
\begin{split}
\text{P}(T_{\text{}}, S_{\text{}}) &= \text{"Rewrite the following text in a "} \\
&\quad + S_{\text{target}} + \text{" style: "} \\
&\quad + T_{\text{original}}
\end{split}
\end{equation}
Upon processing this prompt, a pre-trained Large Language Model (e.g., Llama2) generates a new text \( T_{\text{rewritten}} \) that preserves the content of \( T_{\text{original}} \) but in the style of \( S_{\text{target}} \):
\begin{equation}
T_{\text{rewritten}} = \text{LLM}(\text{Prompt}(T_{\text{original}}, S_{\text{target}}))
\end{equation}
By adapting \( T_{\text{original}} \) to the stylistic nuances of \( S_{\text{target}} \), this stage lays the groundwork for effective style transformation while ensuring the preservation of the original content.



\subsection{\ Second stage with editing approach}

The second stage of the methodology involves a two-step process, focusing on refining and aligning the text with the target style. This stage is crucial for enhancing the style adherence of the rewritten text \( T_{\text{rewritten}} \) from the first stage.

\textbf{Masking method.} The first step employs a fine-tuned RoBERTa-based style classifier\yscomment{Still, how can we use the sequence labeling model to model a single token?}. This classifier is used to assess the stylistic elements of each token in \( T_{\text{rewritten}} \). Let \( t_i \) denote the \( i^{th} \) token in \( T_{\text{rewritten}} \). The style classifier assigns a style score, \( \text{score}(t_i) \), to each \( t_i \). Tokens that fail to meet a predefined stylistic threshold \( v_l \) are marked for revision:
    \begin{equation}
        \text{mask}(t_i) = 
        \begin{cases} 
            \text{[SLOT]} & \text{if } \text{score}(t_i) < v_l \\
            t_i & \text{otherwise}
        \end{cases}
    \end{equation}
Subsequently, contiguous [SLOT] tokens are merged into a single token to optimize the editing process. The resulting masked text is represented as \( T_{\text{masked}} \).

\textbf{Refinement.} In the second step, a fine-tuned BART model is employed for the substitution of [SLOT] tokens in \( T_{\text{masked}} \). The model is trained to recognize and replace these tokens with stylistically appropriate words or phrases. Given \( T_{\text{masked}} \), the BART model generates \( T_{\text{refined}} \), where the [SLOT] tokens are replaced with contextually and stylistically suitable terms:
    \begin{equation}
        T_{\text{refined}} = \text{BART}(T_{\text{masked}})
    \end{equation}
    This process ensures that the final output, \( T_{\text{refined}} \), not only maintains the original content but also aligns closely with the stylistic attributes of \( S_{\text{target}} \).

The combination of these two steps in second stage effectively refines \( T_{\text{rewritten}} \) into a version that is more accurately aligned with the target style. The use of a fine-tuned RoBERTa classifier for initial scoring and masking, followed by a BART model for context-sensitive replacements, exemplifies the unsupervised synthesis approach in achieving precise style alignment.

\subsection{Unsupervised synthesis of stylistic data pairs}

The training of the BART model is a critical component in the style transfer process, particularly in the context of refining and accurately aligning the text with the target style. This section details the methodology and mathematical framework employed in training the BART model.

The BART model is fine-tuned using a dataset where each text instance has been pre-processed by the RoBERTa-based style detector. The detector assesses the style relevance of each token in the original text \( T_{\text{original}} \). Let \( t_i \) represent the \( i^{th} \) token in \( T_{\text{original}} \). A style score, \( \text{score}(t_i) \), is assigned to each \( t_i \) based on its adherence to the target style \( S_{\text{target}} \). The scoring process is defined as:
\begin{equation}
    \text{score}(t_i) = \text{RoBERTa}(t_i, S_{\text{target}})
\end{equation}

Tokens with a style score exceeding a high threshold \( v_h \) are identified for masking. The masking procedure is defined as follows:
\begin{equation}
    \text{mask}(t_i) = 
    \begin{cases} 
        \text{[SLOT]} & \text{if } \text{score}(t_i) > v_h \\
        t_i & \text{otherwise}
    \end{cases}
\end{equation}
In instances where [SLOT] tokens occur consecutively, they are merged into a single token to facilitate efficient training and subsequent text generation.

The fine-tuning of the BART model is then conducted using these pre-processed text instances. The training process involves feeding the model with texts containing [SLOT] tokens, with the objective of teaching the BART model to generate stylistically appropriate replacements. The training objective can be expressed as\yscomment{In this case, we may masked consecutive tokens but we can only generate a single token? Does it mean we can only shorten the sentence during revision, but this is not reasonable?}:
\begin{equation}
    \text{Minimize } \mathcal{L}(\text{BART}(T_{\text{masked}}), T_{\text{original}})
\end{equation}
where \( \mathcal{L} \) is a loss function measuring the difference between the BART-generated text and the target text \( T_{\text{original}} \) in terms of style alignment and contextual relevance.

Through this training process, the BART model learns to generate text that not only fills the [SLOT] with contextually appropriate content but also ensures that these replacements are closely aligned with the desired style \( S_{\text{target}} \). This results in a model capable of effectively contributing to the sophisticated style transfer process outlined in the earlier stages of this methodology.

